ChatEDA: A Large Language Model Powered Autonomous Agent for EDA

The integration of a complex set of Electronic Design Automation (EDA) tools to enhance interoperability is a critical concern for circuit designers. Recent advancements in large language models (LLMs) have showcased their exceptional capabilities in natural language processing and comprehension, offering a novel approach to interfacing with EDA tools. This research paper introduces ChatEDA, an autonomous agent for EDA empowered by an LLM, AutoMage, complemented by EDA tools serving as executors. ChatEDA streamlines the design flow from the Register-Transfer Level (RTL) to the Graphic Data System Version II (GDSII) by effectively managing task decomposition, script generation, and task execution. Through comprehensive experimental evaluations, ChatEDA has demonstrated its proficiency in handling diverse requirements, and our fine-tuned AutoMage model has exhibited superior performance compared to GPT-4 and other similar LLMs.

==> doc/bio.tex <==
\vspace{-.4in}
\begin{IEEEbiography}
    [{\includegraphics[height=1.26in,clip,keepaspectratio]{./avatar/haoyuan}}]
    {Haoyuan Wu} received his B.Eng. degree in Software Engineering from Sun Yat-Sen University (SYSU) in 2022 and an MSc. degree in Computer Science from The Chinese University of Hong Kong (CUHK) in 2023. He is currently a researcher at the Shanghai Artificial Intelligence Lab. His research interests include large language models, machine learning, and electronic design automation.
\end{IEEEbiography}

\vspace{-.4in}
\begin{IEEEbiography}
    [{\includegraphics[height=1.26in,clip,keepaspectratio]{./avatar/leon}}]
    {Zhuolun He}
	received his Ph.D.~degree from the Chinese University of Hong Kong (CUHK) in 2023, and his B.S.~degree in computer science and engineering from Peking University in 2017. He is currently a postdoctoral fellow at the Department of Computer Science and Engineering, CUHK.
\end{IEEEbiography}

\vspace{-.4in}
\begin{IEEEbiography}
    [{\includegraphics[height=1.26in,clip,keepaspectratio]{./avatar/xinyun}}]
    {Xinyun Zhang}
	received his B.Eng.~degree from the School of Electrical Engineering, Xi'an Jiaotong University, in 2018, and his M.S.~degree from the School of Engineering, The Hong Kong University of Science and Technology, in 2020. He is currently pursuing the Ph.D degree with the Department of Computer Science and Engineering, The Chinese University of Hong Kong. His current research interests include computer vision and machine learning.  
\end{IEEEbiography}

\vspace{-.4in}
\begin{IEEEbiography}
    [{\includegraphics[height=1.26in,,clip,keepaspectratio]{./avatar/xufeng}}]
    {Xufeng Yao}
    received his B.Eng. degree in Information System and Information Management from Fudan University (FDU) in 2016 and an MSc. degree in Computer Science from The Chinese University of Hong Kong (CUHK) in 2020. He is currently pursuing his Ph.D. degree at the Department of Computer Science and Engineering, The Chinese University of Hong Kong. His research interests include computer vision and machine learning.
\end{IEEEbiography}

\vspace{-.4in}
\begin{IEEEbiography}
    [{\includegraphics[height=1.26in,clip,keepaspectratio]{./avatar/su-zheng}}]
    {Su Zheng} received his B.Eng. degree from Fudan University in 2019, and his M.S. degree from Fudan University in 2022. 
    He is currently pursuing his Ph.D. degree at the Department of Computer Science and Engineering, the Chinese University of Hong Kong (CUHK), under the supervision of Prof.~Bei Yu and Prof. Martin D.F. Wong. 
    His research interest is to solve critical problems in electronic design automation (EDA) with advanced artificial intelligence (AI) methods. 
\end{IEEEbiography}

\vspace{-.4in}
\begin{IEEEbiography}
    [{\includegraphics[height=1.26in,clip,keepaspectratio]{./avatar/haisheng}}]
    {Haisheng Zheng} is currently a Researcher at Shanghai AI Laboratory, since 2022. From 2020 to 2022, he was a Research and Development Engineer at SmartMore. His research interests include artificial intelligence, embedded systems, high performance compute, and IC design.
\end{IEEEbiography}

\vspace{-.4in}
\begin{IEEEbiography}
    [{\includegraphics[height=1.26in,clip,keepaspectratio]{./avatar/byu}}]
    {Bei Yu}
    (M'15-SM'22)
    received the Ph.D.~degree from The University of Texas at Austin in 2014.
    He is currently an Associate Professor in the Department of Computer Science and Engineering, The Chinese University of Hong Kong.
    He has served as TPC Chair of ACM/IEEE Workshop on Machine Learning for CAD, and in many journal editorial boards and conference committees.
    He is the Editor of IEEE TCCPS Newsletter.
    He received ten Best Paper Awards from IEEE TSM 2022, DATE 2022, ICCAD 2021 \& 2013, ASPDAC 2021 \& 2012, ICTAI 2019, Integration, the VLSI Journal in 2018,
    ISPD 2017, SPIE Advanced Lithography Conference 2016, and six ICCAD/ISPD contest awards.
\end{IEEEbiography}


